Robot Learning in Homes: Improving Generalization and Reducing Dataset Bias

Data-driven approaches to solving robotic tasks have gained a lot of traction in recent years. However, most existing policies are trained on large-scale datasets collected in curated lab settings. If we aim to deploy these models in unstructured visual environments like people's homes, they will be unable to cope with the mismatch in data distribution. In such light, we present the first systematic effort in collecting a large dataset for robotic grasping in homes. First, to scale and parallelize data collection, we built a low cost mobile manipulator assembled for under 3K USD. Second, data collected using low cost robots suffer from noisy labels due to imperfect execution and calibration errors. To handle this, we develop a framework which factors out the noise as a latent variable. Our model is trained on 28K grasps collected in several houses under an array of different environmental conditions. We evaluate our models by physically executing grasps on a collection of novel objects in multiple unseen homes. The models trained with our home dataset showed a marked improvement of 43.7% over a baseline model trained with data collected in lab. Our architecture which explicitly models the latent noise in the dataset also performed 10% better than one that did not factor out the noise. We hope this effort inspires the robotics community to look outside the lab and embrace learning based approaches to handle inaccurate cheap robots.

==> extra.tex <==
\subsection{Grasp Data Collection}
We collected a diverse set (see Fig \ref{fg:train_data}) of planar grasping and pushing data in 6 homes in various environments using multiple robots. The framework is summarized in Algorithm~\ref{alg:data_collection}. When experiments are conducted in the lab, the environment can be curated (e.g. using green cloth, white background) such that heuristic methods like background color subtraction/segmentation/thresholding could be used for object pose estimation. However, since we are collecting data in homes which have very unstructured visual input, we used an object detector (specifically tiny-YOLO, due to compute and memory constraints in the low cost arm) \cite{redmon2016yolo9000}. It gave decent bounding box predictions for the objects amidst clutter and diverse backgrounds, of which we only use the 2D location and discard the object class information. Once we have the 2D location, we first sample a grasp and then run RANSAC on the noisy object PointCloud to estimate the 3D grasp location. Motion planning was also a challenge since our under-constrained robot only has 5 DOFs. When collecting training data, we scattered a diverse set of objects and let the mobile base randomly move and grasp objects. The base was constrained to a 2m wide area to prevent the robot from colliding with obstacles beyond its zone of operation. To bootstrap learning, we used epsilon-greedy exploration and sampled grasps from a pre-trained model \cite{pinto15}. We collected a dataset of about 28$K$ grasps. 

\begin{algorithm}
\caption{Data Collection in Homes}
\label{alg:data_collection}
\begin{algorithmic}
\State Initialize robot arm/base, motion planner $\mathcal{P}$, grasp sampler $\mathcal{G}$ and object detector $\mathcal{D}$
\While {NoCollisionDetected and ObjectsExists and BaseWithinZoneLimits}
    \State With probability $\epsilon_{near}$, select action $a_t$ to grasp closeby, otherwise move base
    \If {$a_t$ is grasp closeby} {
        \State Capture entire scene image $I_{close}$; detect set of nearby objects $O_{close}=\mathcal{D}(I_{close})$
        \State Estimate 3D positions of $O_{close}$ from noisy PointCloud with RANSAC
        \For {object $o$ = 1:$|K|$ where $K = \{x | x \in O_{close}, \exists \mathcal{P}(x)\}$}
            \State Capture image patch around object $I_{o}$; sample grasp $g_{o} \sim \mathcal{G}(I_{o})$; execute $g_{o}$ 
        \EndFor
    }
    \Else
        \State Detect objects further away $O_{far}=\mathcal{D}(I_{far})$; Compute 3D position;
        \State Sample pose to move to from distribution $p_t \sim O_{far}$; move base to $p_t$
        \State Assign $a_{t+1}$= grasp closeby; if no objects detected, \textbf{exit}
    \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsection{Planar Push Data Collection}
For collecting push data, we implemented the approach in \cite{pulkitpoking}. Given the object position in image space, a random direction and length was computed for the planar push and applied on the robot. We collected about 4$K$ pushes in homes and in lab. 

\begin{figure*}[t]
\centering
\includegraphics[width = 0.92\linewidth]{figures/dataset.pdf}
%   \vspace{-0.1in}
\caption{Selected grasps from data collected in the homes and lab data from \cite{pinto15}. The attempted planar parallel-jaw grasps are also plotted on each image.}
%   \vspace{-1.5em}
\label{fg:train_data}
\end{figure*}
